Hidden Connections: Tracing the BCG Stellar Mass-Halo Mass Relation in the SDSS-GalWCat19 Cluster Catalog

The stellar-to-halo mass (SMHM) relation of brightest cluster galaxies (BCGs) provides key insight into the connection between BCG growth and the assembly of their host halos. We analyze this relation using the spectroscopic SDSS GalWCat19 cluster catalog, selecting 996 systems with log(M200) >= 13.6, log(Mstar) >= 10.5, and 0.02 <= z <= 0.125 to limit evolutionary effects and ensure stellar-mass completeness. We fit lognormal scaling relations with a Markov Chain Monte Carlo (MCMC) framework that accounts for measurement uncertainties and intrinsic scatter. For the fiducial SMHM relation, <log Mstar | M200> = alpha + beta log(M200/Mpiv) with log(Mpiv) = 14.2, we find a shallow slope beta = 0.17 +/- 0.03, normalization alpha = 11.04 +/- 0.01, and intrinsic scatter sigma_int = 0.19 +/- 0.01 dex. Recasting the relation in normalized form reduces the scatter to 0.16 +/- 0.01 dex, while including the magnitude gap M14 further reduces it to 0.14 +/- 0.01 dex. Variations in richness, redshift, and mass thresholds produce systematic shifts that are small compared to the statistical uncertainties, indicating that our inferred relations are robust to plausible selection choices. The reduced scatter when including M14 supports a picture in which BCG stellar mass reflects both halo mass and halo assembly history.

==> name.tex <==
\begin{thebibliography}{}
\bibitem[de Lucia \& Blaizot(2007)]{deLucia2007} de Lucia, G., \& Blaizot, J. 2007, MNRAS, 375, 2
\bibitem[Lidman et al.(2012)]{Lidman2012} Lidman, C., Suherli, J., Muzzin, A., et al. 2012, MNRAS, 427, 550
\bibitem[Zhang et al.(2016)]{Zhang2016} Zhang, Y., Yu, H., \& Ho, L. 2016, ApJ, 817, 119
\bibitem[Lin \& Mohr(2004)]{LinMohr2004} Lin, Y.-T., \& Mohr, J. J. 2004, ApJ, 617, 879
\bibitem[Kravtsov et al.(2018)]{Kravtsov2018} Kravtsov, A. V., Vikhlinin, A., \& Meshcheryakov, A. 2018, Astronomy Letters, 44, 8
\bibitem[Henden et al.(2020)]{Henden2020} Henden, N. A., Puchwein, E., Saro, A., et al. 2020, MNRAS, 498, 1576
\bibitem[Lin et al.(2017)]{Lin2017} Lin, Y.-T., Mandelbaum, R., Huang, H.-J., et al. 2017, ApJ, 851, 139
\bibitem[Golden-Marx et al.(2019)]{GoldenMarx2019} Golden-Marx, J. B., Miller, C. J., et al. 2019, ApJ, 878, 6
\bibitem[Rykoff et al.(2014)]{Rykoff2014} Rykoff, E. S., Rozo, E., Busha, M. T., et al. 2014, ApJ, 785, 104
\bibitem[Muzzin et al.(2012)]{Muzzin2012} Muzzin, A., Wilson, G., Yee, H. K. C., et al. 2012, ApJ, 746, 188
\bibitem[Sifón et al.(2015)]{Sifon2015} Sifón, C., Hoekstra, H., Cacciato, M., et al. 2015, A\&A, 575, A48
\bibitem[YourReferenceGalWCat()]{YourReferenceGalWCat} Your Reference for GalWCat catalog, YYYY, Journal, Volume, Page
\end{thebibliography}
